Hierarchical Fine-Grained Image Forgery Detection and Localization

Differences in forgery attributes of images generated in CNN-synthesized and image-editing domains are large, and such differences make a unified image forgery detection and localization (IFDL) challenging. To this end, we present a hierarchical fine-grained formulation for IFDL representation learning. Specifically, we first represent forgery attributes of a manipulated image with multiple labels at different levels. Then we perform fine-grained classification at these levels using the hierarchical dependency between them. As a result, the algorithm is encouraged to learn both comprehensive features and inherent hierarchical nature of different forgery attributes, thereby improving the IFDL representation. Our proposed IFDL framework contains three components: multi-branch feature extractor, localization and classification modules. Each branch of the feature extractor learns to classify forgery attributes at one level, while localization and classification modules segment the pixel-level forgery region and detect image-level forgery, respectively. Lastly, we construct a hierarchical fine-grained dataset to facilitate our study. We demonstrate the effectiveness of our method on $7$ different benchmarks, for both tasks of IFDL and forgery attribute classification. Our source code and dataset can be found: \href{https://github.com/CHELSEA234/HiFi_IFDL}{github.com/CHELSEA234/HiFi-IFDL}.

==> section/figure_table_latex/figure_res_localization.tex <==
\begin{figure*}[t]
    \centering
    \begin{overpic}[width=0.95\textwidth]{results/loc_figure}
    \put(-1,27.5){Image}
    \put(1,19){\small{GT}}
    \put(-0.5,12.5){\small{PSCC}}
    \put(0.5,10.5){\small{\cite{liu2022pscc}}}
    \put(0,4){\small{Ours}}
    \end{overpic}
    \vspace{-2mm}
    \caption{Comparison of qualitative results on different forged images. The first $6$ columns are from image editing methods whereas the last $3$ columns are images generated by Faceshifer~\cite{li2019faceshifter} and STGAN~\cite{liu2019stgan}.}
    \label{fig_viz_manipulation}
\end{figure*}
